Asynchronous Perception Machine For Efficient Test-Time-Training

In this work, we propose Asynchronous Perception Machine (APM), a computationally-efficient architecture for test-time-training (TTT). APM can process patches of an image one at a time in any order asymmetrically and still encode semantic-awareness in the net. We demonstrate APM's ability to recognize out-of-distribution images without dataset-specific pre-training, augmentation or any-pretext task. APM offers competitive performance over existing TTT approaches. To perform TTT, APM just distills test sample's representation once. APM possesses a unique property: it can learn using just this single representation and starts predicting semantically-aware features. APM demostrates potential applications beyond test-time-training: APM can scale up to a dataset of 2D images and yield semantic-clusterings in a single forward pass. APM also provides first empirical evidence towards validating GLOM's insight, i.e. input percept is a field. Therefore, APM helps us converge towards an implementation which can do both interpolation and perception on a shared-connectionist hardware. Our code is publicly available at this link: https://rajatmodi62.github.io/apm_project_page/.

==> sections/broader_impact.tex <==
\section{Broader Impact}

   
    Kolmogorov-Arnold superposition theorem\footnote{It solves a constrained version of hilbert's thirteenth problem \cite{hinton2023represent}} states that a continuous signal can be broken down into linear combinations of several basis functions multiplied by some coefficients\cite{modi2017steganography}. GLOM's mathematical analogy involves combining information coming from many different locations. In SPM, the trigger column T contains an entangled signal and acts as an encoding operation. It can also be considered to be a tape being fed to a machine\cite{turing1936computable}. The unfolding process is equivalent to disentangling a different signal for every location. The shared neural field acts as a decoder/write head. Binding is done via the positional encoding now\cite{hinton2023represent}. All the neurons of SPM are trying to do \textit{one job} only: explain the existence of \textit{a single object} vector at a particular location. We believe that it shall help make progress towards \emph{eliminating} the  binding problem\cite{hinton2023represent, greff2020binding, lowe2024rotating, chalmers1995facing, crick2003framework}. 
    
    
    
    
    
    
    
    
   



==> sections/future_work.tex <==
\section{Further Work}
The comments in this section are the sole opinion of the author. It might be taken with a grain of salt and suspicion: for it is mere philosophy and has not been built into machines (yet).

\subsection{On Oversampled Positional Fields}
Transformers managed to become resolution-independent by choosing a large image size and pasting a smaller image into it\cite{carion2020end}\footnote{CNNs did this by via full convolutions\cite{long2015fully} because MLPs had the restriction of constant number of input neurons which could not be mapped to different image sizes. We have removed this now since input neurons of a MLP are now the dimensions of the column query. It has nothing to do with the number of input columns anymore. Finally, in MLP a neuron at a higher layer is connected to every neuron is lower layer, so that little guy knows whatever happens to the neurons below him.\cite{vaswani2017attention}}. Attention layers then typically mask the inputs which need not be attended to. However, masked regions still consume memory\footnote{Basic linear algebra says that a matrix can be divided into smaller matrices whose multiplication can then be split across cores since multiplication is a recursive property. The results are then collected across workers. Column queries make sure that each core is processing multiplications of a useful input percept and not a masked token.}. Using column queries, it becomes possible to entirely bypass this: One can now create column queries at a significant higher resolution by repeating them many times. \textit{Only} the queries which cover the spatial span of the pixels of an input image need to be fired into the MLP. This shall save on the queries which are not required, and facilitate faster training of the machine. Note that attention \textit{cannot} do this, since a batch during forward pass needs to be kept at a \textit{fixed} resolution for splitting matrix-multiplication across parallel cores of a gpu. In our case, all the patches no matter of what resolution have become a batch. This batch of columns is now same as the batch of rays we typically fire into the neural fields. 

\subsection{On binding columns to objects at MLP input}
Earlier object detectors built ROI proposals at encoder input. ROI regions were treated as a batch. Later, object queries were shifted to do cross attention from encoder: a neural net learnt parameters to retrieve relevant objects from an encoder's associative memory. Next, observe neural fields \cite{yu2021unsupervised}: slots can selectively bind to input rays of the same object at input. If one knows in advance which rays correspond to which object, only those rays are fired into the neural field to retrieve objects. Now that 2D perceptual symmetry has been broken, object awareness could be built into the column queries by iterative forms of self-attention. This then reduces to the standard GLOM architecture proposed by \cite{hinton2023represent} which relies on columns. (our column queries are similar to that). Object-awareness should emerge in upper levels of the column hierarchy itself thereby helping our community move towards a more GLOM-based net.\cite{hinton2023represent} However, it will still face memory issue \cite{modi2023occlusions} since all columns would need to be kept in the memory.

\subsection{On visualization mechanisms in neural nets}
How should one visualize the representations in a neural net? One way is to estimate which neuron responds to which input signal the most. However, the net needs several forward passes in this case. Second way is to visualize attention maps of individual heads in an attention layer. However, if we accept the object-binding property\cite{greff2020binding}, i.e. each attention head specializes for one object, then what happens when the number of objects in the scene are far more than the number of heads in an attention layer? A third way is to take dot product of the feature vector in one location of an input percept with all the vectors in another percept. This is $O(N^4)$ x
operation for all locations which is costly to compute. The visualization mechanism by \cite{modi2023occlusions} is far simpler: simple t-sne reduction between all vectors of the same percept readily reveals islands which a network has learnt. \emph{One can then readily see islands of background objects also, which otherwise might have been classified as "stuff" and "background"\cite{kirillov2019panoptic} OR treated as a component of PCA reduction that could be discarded}.\footnote{One can try a simple experiment. Take an image with one person and a cluttered background. Try thresholding first PCA component in a feature obtained from DINOv2. You will find full background cannot be removed, or that the network removes the whole person whereas it should have removed the background.}



==> sections/glom_connection.tex <==
\section{Differences from GLOM}
GLOM is a very inspiring philosophical paper for our community. All the technical aspects mentioned in this section refer to the open source Github implementation\cite{glom_pytorch} of GLOM which has been widely accepted.\footnote{Papers using the same repository have been published in peer-reviewed conferences i.e, CVPR. \cite{garau2022interpretable}}. However, there are several crucial differences. 

% We got some of whose ideas working on realistic datasets like COCO\cite{lin2014microsoft}. 

Firstly, in GLOM the columns were the weights of a neural net. In our case, the columns are the actual contents of an input image (the only learnt parameters are that of a single CNN filter). Secondly, GLOM assumes that each column sees only a part of an input image as an input. We found this not to work as well as allowing all the columns to have all the image features common to them (like DNA) for the machine has difficulty breaking RGB symmetry and making columns significantly different from each other. Third, GLOM assumes that islands of agreement emerge by competing rounds of attention in stacked columns. In our case, all the columns are iid in accordance with Lemma 1. \emph{This was needed to bypass the memory law}. Perception can still occur since the net is shared across locations of the input. Fourth, the positional encoding added to all columns in GLOM is parametric. This does not guarantee that the neural net learns correct ordering information among columns injected into the network. In our architecture, we use hardcoded non-parameteric positional encoding. Note that this is in line with how the best variants of DETR \cite{carion2020end} use hard-coded positional encodings during encoding instead of learnt parametric encodings.
Finally, GLOM assumes that columns emerge by self-supervising the architecture via objectives like reconstruction. In our architecture, we find that doing dense feature level supervision at each image location works allows islands predicted by MLP to align with islands predicted by DINO. This exploits the fact that islands at topmost levels already exist in transformers\cite{modi2023occlusions}, and dense column-based features can be distilled readily into a neural field \cite{wang2022clip}\footnote{Models like PixelNERF\cite{yu2021pixelnerf} inject image latent in input and predict rgb and alpha. We estimate an inverse function: given the location of rgb patch of an image, what will be the higher dimensional feature (islands) and rgb corresponding to it.}. We found it more beneficial for a MLP to predict higher dimensional features than merely predicting RGB values: although the higher dimensional space has a significant entropy due to higher degrees of freedom, our $L_2$ loss between predicted column-vectors and vectors distilled from DINO more than compensates for those margins of error. 

\textbf{Can part-whole hierarchies be learnt using our architecture?}  Our neural net operates at extreme ends of the part-whole hierarchy, it predicts both lower level rgb and higher object-level features. Among other levels of hierarchy, GLOM still assumes a certain degree of agreement. \textit{If} multi-level agreement could be made to emerge, then we could interpret the column vector $v_c$ as just a cascade of smaller vectors at individual levels of the hierarchy at a particular image location. We could then memorize this bigger vector by just increasing the count of neurons in the last layer of our MLP. This is in agreement with how standard neural fields typically just memorize the entire radiance field. 





==> tables/ablations/ablation_aug.tex <==

% \begin{table}[h]
% \centering
% \caption{Augmentation \textit{harms} SPM. Learning from a single distilled token is best. It provides a clean supervisory signal to SPM towards an optimal point in the optimization landscape. }
% \label{tab:aug_effect}
\begin{tabularx}{\linewidth}{l|l|l}
% \begin{tabular}{l|l|l}
 & w/o aug & w aug \\
\hline
SPM   & \textbf{98.6}  & 76.7
\end{tabularx}
% \end{table}

==> tables/ablations/ablation_conv_count.tex <==

% \begin{table}[h]
% \centering
% \caption{Increasing number of convolutions from 1 to 3 in trigger column T improves performance of SPM. }
% \label{tab:conv_effect}
\begin{tabularx}{\linewidth}{l|l|l}
 & $T_{c1}$ & $T_{c3}$ \\
\hline
SPM   & 96.08  & \textbf{97.67}
\end{tabularx}
% \end{table}
